parRSB: Exascale Spectral Element Mesh Partitioning

We introduce parRSB - a parallel, highly scalable graph partitioner for spectral element meshes that produce high quality partitions. parRSB is based on Recursive Spectral Bisection (RSB) algorithm implemented on the dual graph of the input mesh. RSB uses the Fiedler vector, which is the eigenvector associated with the smallest non-zero eigenvalue of the Laplacian matrix of the dual graph for making partitioning decisions and tries to minimize the communication volume between the partitions. We implemented two numerical methods: Lanczos, and Inverse iteration using Conjugate Gradient method to compute the Fiedler vector. We present partitioning results using parRSB on Summit and Frontier supercomputers at Oak Ridge National Laboratory to illustrate the quality of the partitions produced by parRSB and the scalability of our implementation. We also present results for some of the optimizations we did to speed up the partitioning process.

==> tex/csr.tex <==
\subsection{CSR Representation}\label{subsec:csr_laplacian}

Each element of the mesh is associated with a row in the Laplacian matrix.
If the total number of elements of the mesh is $m$, the Laplacian $\mathbf{L}$
will be a $m \times m$ sparse matrix.
If we are using $P$ processors in parallel for partitioning, each processor will
have $m_r \approx \frac{m}{P}$ elements of the mesh and hence $m_r$ rows of the
Laplacian.
To ensure load balance, the elements are distributed such that the maximum difference
of $m_r$ between any two processors is 1.
Rows can be numbered similar to the elements in the mesh such that row $e$ corresponds
to the element with global element id $e$.
Each nonzero entry in a row, except when it falls on the diagonal of the matrix,
denotes a connection between element $e$ and adjacent elements in the mesh.
So the total number of nonzeros in a given row, not
counting the diagonal, is equal to the number of neighbors of the corresponding
element.
In the case of unweighted Laplacian, the value of all off-diagonal nonzeros is $-1$.
In the case of the weighted Laplacian, each entry is equal to the number of vertices
shared with the corresponding adjacent element.
In both of these cases, it is required to identify neighbors of elements.

Each element in a SEM mesh is represented by a set of $u$ vertices which are numbered
globally.
Vertices that have the same physical coordinates will have the same global number.
\footnote{PDEs with periodic boundary conditions can also have shared global vertices
that are not physically coincident.}
We use this global numbering to identify neighbors of an element as two neighbor elements
should at least share one vertex, meaning that their local graphs have at least one global
number in common.

Consider a local vertex $v_{i}^e, 1 \le i \le v$ in an element with a global
element number $e$.  Unlike vertices, elements are not duplicated across
processors.  So let's assume that element $e$ is in processor $p_{e}$ where $1
\le p_{e} \le P$.
So each element $e$ has a unique processor id associated with it.
To find the elements which share local vertex $v_i^e$, we send the tuple
$(v_{i}^{e}, e, p_{e})$ to the processor with rank $(v_{i}^{e} \bmod P) + 1$.
$v_{i}^{e}$ is the global number of the local vertex $v_i$ of $e$.
This generalized all-to-all exchange can be executed in only $\log_2 P$
communication phases.

After the exchange, all the tuples that share the same global id $v_{i}^{e}$
will end up in the same processor.
Now we can find the set of elements which share the vertex $v_{i}^{e}$ and the
set of processors where those vertices reside.
Let the set of elements that share vertex $v_{i}^{e}$ be $E_{v_{i}^{e}}$ and the
set of processors on which they reside be $P_{v_{i}^{e}}$.
We now send the set of tuples $\{(v_{i}^{e}, e) \mid e \in E_{v_{i}^{e}}\}$
to each member of $P_{v_{i}^{e}}$.
Upon the reception of these tuples, each processor can now construct a map between
a global vertex number $v_{i}^{e}$ and the set of elements in which it is a part of.
Then the set of neighbors of an element can be constructed by taking the union of
$n_v$ sets corresponding to the vertices of the element.

For the unweighted Laplacian, we are simply interested in distinct neighbors
of an element but for the weighted Laplacian we count how many times each element
shows up in the neighbor list as well.
If element $e_j$ shows up in global element $e_i$'s neighbor list, entry
$l_{ij}$ of the Laplacian will be non-zero and its value is set based on
whether we use weighted or unweighted Laplacian.

All of the non-zero values local to a processor can now be converted to CSR format
which gives us a distributed CSR matrix.
For each non-zero value, we create a tuple $(e_i, e_j, l_{ij})$ where $e_i, e_j$
are the global element numbers corresponding to the row and column id in the Laplcain
matrix.
$l_{ij}$ is defined as in Section~\ref{sec:rsb}.
We now sort these tuples first by $e_i$, then by $e_j$.
This is the order in which the column indices $e_j$ and non-zero values $l_{ij}$
appear in the CSR matrix.
We now set $n_r$ to be the distinct $e_i$ values which is the distinct number of
rows owned by each processor locally.
We now only need to store start and end of each row in a separate data structure
for the purposes of indexing to the start and end of each row.
This is necessary since evaluating Laplacian for a given input vector
$\underline{x}$ is equal to evaluating the dot product of $\underline{x}$ with
each row of the Laplacian.

In order to evaluate $y = \mathbf{L} \underline{x}$ when $\mathbf{L}$ is
row-distributed (i.e., approximately $n/P$ rows on each processory, with
each row $e$ of $\mathbf{L}$ is contiguous within processor $p_e$),
required input values from $\underline{x}$ need to be gathered on each
processor.
This is necessary because the input vector $\underline{x}$ is
partitioned across processors according to the same distribution as
the columns of $\mathbf{L}$.
Since each local row of the Laplacian matrix is doing a dot product with the
input vector $\underline{x}$, we need to gather the $\underline{x}$-values that
correspond to the nonzero column ids of the local CSR matrix.

Suppose we have, on average $n_z$ non-zeros per row in the Laplacian matrix.
This means, each rank has to store $n_r + 1$ integers for indexing the rows,
$n_r \times n_z$ longs for storing column ids and $n_r \times n_z$ doubles
for the $l_{ij}$ values.
If we are using the unweighted Laplacian, except for $n_r$ values that falls on
the diagonal, all the other $l_{ij}, i \ne j,$ values are equal to $-1$.
So we should be able to get by just storing $n_r$ doubles for the diagonal $l_{ij}$
values instead of $n_r \times n_z$.
The same is true for the weighted Laplacian except that the non-diagonal
entries $l_{ij}, i \ne j,$ can now be either $-1, -2$ or $-4$ based on the
connection type between the elements $i$ and $j$.


==> tex/disconnected.tex <==
\section{Detect and Repair Disconnected Components}

Disconnected sub-graphs can show up as we go down the RSB bisection tree and can degrade
the convergence rates of numerical methods used to find the fiedler vector.
Disconnected components can be detected by doing a Breadth First Search (BFS) in the
tentative sub-graphs (partitions) before bisection.
In each sub-graph, we start by assigning value 1 to a random vertex and all the vertices
that can be reached from this vertex using BFS.
If there are un-assigned vertices left after BFS, then we have disconnected components.
We assign value 2 to a random vertex from these un-assigned vertices and all the vertices
that can be reached from it using BFS.
We keep doing this separately in each sub-graph till we assign a number to all the
vertices in respective sub-graphs.
Vertices that are assigned the same number forms a component.
Then we pick the component with the smallest number of vertices in any of the sub-graphs.
Suppose the smallest componet was found on sub-graph A.
We then send that entire component to the sub-graph B.
This creates a load imbalance and we transfer enough elements from the element interface
of two sub-graphs to sub-graph A.
We do this process multiple times to see if that can repair the disconnectivity.
This may not always be possible since there may not be enough elements in the interface
to account for the load imbalance.
If that is the case, we forget about the repair and simply proceed with load balanced
partitions.


==> tex/intro.tex <==
\section{Introduction}\label{sec:intro}

With leadership class computing facilities commissioning powerful computers
that are getting closer to exascale, users of these facilities are trying to
solve much harder and larger problems as fast as possible.
There are numerous challenges faced by users in adapting their code, algorithms
and workflow in preparation for future exascale systems.
Looking at state of the art pre-exascale systems in the U.S., we can see that
these systems increasingly use accelerators or General Purpose Graphic Processing
Units (GPGPUs).
Developing scalable algorithms and implementing them efficiently on these systems is a
challenging task, partly due to complicated memory hierarchies of GPGPUs and
the complexity of programming models involved.
With exascale computers reaching hundreds of thousands of processors, users also
have to pay extra attention to how to communicate efficiently among different
processors in these distributed memory parallel computers.

In the context of scientific simulations, efficient communication has multiple
advantages.  Many scientific simulations start with reading a \textit{mesh},
which is a representation of the computational domain using smaller regions
called \textit{elements}.  The next step is to distribute these elements among the
processors. This element distribution is known as {\em partitioning} and is
critical to the overall efficiency of the simulation.  Exascale mesh
partitioning comes with its own challenges mainly due to the size of the
problem and the level of parallelism.  Large spectral element simulations with
$10^8$--$10^9$ elements are already running on pre-exascale systems like Summit
at OLCF, which is a sign that we will see meshes with $10^9$--$10^{10}$ elements
on exascale machines that are planned for future.

There are two important properties which affect the parallel efficiency at
scale in distirbuted memory parallel programs: \textit{load balance} and
\textit{inter-processor communication}.  It is desirable to have load
distributed evenly among all the processors.  If each of the processors has
enough work to offset the communication cost, then load balance is the most
important metric affecting the parallel
efficiency of the simulation.  If the work is not well balanced, every
processor will be as slow as the one with the most work since other processors
have to wait for the slowest processor at sync points.

If a user wants to run faster (reduced time-to-solution) by using as many
processors as possible while retaining reasonable parallel efficiency, then it
is important to minimize the time spent in communication among different
processors.  This is because with an increased processor count the work per
processor is smaller and, after a certain point, the communication costs
can dominate the work allocated to the processor.  A \textit{good} partition
should minimize a selected communication metric based on the communication
pattern of the application and the network characteristics
so that the parallel efficiency is preserved at scale.  There are multiple ways
to assess communication cost and we will define metrics which measure multiple
aspects of communication in Section~\ref{sec:results}.

The amount of time a user is willing to spend on finding a partition also
depends on the application domain as well as the desired quality of the
resulting partition.  If the time taken for partitioning is only a fraction of
the time the actual application is run, then the savings of runtime by having a
good partition will offset the time spent on finding it.  This is in general
true for most scientific simulations where partitioning is done only once in
the beginning while simulation runs might take weeks to complete.  However, in
Adaptive Mesh Refinement (AMR) or in Very Large-Scale Integration (VLSI) design
processes, it is more beneficial to have a faster partitioning algorithm than a
one which results in higher quality partitions~\cite{buluc16,klmh11}.

In spectral/finite element simulations (SEM/FEM), the computational domain
(mesh) is represented by a collection of \textit{elements} which are in turn
represented as a set of vertices. The mesh topology can be represented as a
graph, $H(V_H, E_H),$ where $V_H$ is the set of vertices and $E_H$ is the set of
edges connecting vertices forming elements and their connectivity.  Each
element in the mesh is represented by $n_v$ vertices from $V_H$.

Different types of elements are used in FEM and SEM computations based on the
problem dimension and desired trade off between ease of modelling and
computational efficiency.  Our primary focus is partitioning 3D hex meshes and
2D quad meshes although the methods we developed can be easily extended to
other element types in 2D and 3D.  In 2D, if we are using quad elements, $n_v =
4$ and for hex elements in 3D, $n_v = 8$.

Since we want to partition the elements to processors, not the vertices, we
consider the dual graph $G(V, E)$ of $H$.  Here $V$ is the set of vertices of
dual graph $G(V,E)$ where each vertex represents a spectral or finite
element made up of $n_v$ vertices from $V_H$.  $E$ is the set of connections
(edges) between elements.  Edges exist between elements that share a vertex,
edge, or face.

Given a graph $G(V, E)$ and the numper of processors $P$ with non-negative edge
weights $\omega : E \rightarrow \mathbb{R}_{>0}$, the graph partitioning problem
as it relates to mesh partitioning is to find a set of subsets $V_1, V_2, \dots V_P$,
such that:
\begin{enumerate}
  \item $V_1 \cup V_2 \cup \dots V_P = V$
  \item $V_i \cap V_j = \emptyset,\,\, i \ne j,\, 1 \le i, j \le P$
\end{enumerate}
We additionally put a constraint on the size of the partitions $V_i$ in order
to produce load balanced partitions,
\begin{eqnarray} \label{eq:balance}
   \max{\{\mid V_i \mid - \mid V_j \mid\}} = 1,\,\,1 \le i, j \le P, 
\end{eqnarray}
where $\mid V_i \mid$ is the size of the subset $V_i$.

% {\bf [Some work here...]}
% Spectral Element community built around Nek5000, a fast and scalabale open
% source CFD solver, has been using genmap, a serial Recursive Spectral Bisection
% (RSB) partitioner.
% With larger meshes, we found the serial implementation to be a bottleneck for
% users of Nek5000 since it was taking a longer time to produce the partitions.
% \textit{parRSB} is the parallel implementation of genmap that is based on
% Message Passing Interface (MPI) for parallelizing across multiple cores (ranks,
% processors) of distributed memory parallel computers.
% In this paper we describe in detail how we adapted Recursive Spectral Bisection
% algorithm to run at scale on leadership class computers.

The remainder of the paper is organized as follows.
We look at the related work in Section~\ref{sec:related} followed by a description
of our approach Sections~\ref{sec:rsb}--\ref{sec:inverse}.
We present results in Section~\ref{sec:results} followed by a discussion
of future directions in Section~\ref{sec:future}.

